On Tradeoffs in Learning-Augmented Algorithms

The field of learning-augmented algorithms has gained significant attention in recent years. These algorithms, using potentially inaccurate predictions, must exhibit three key properties: consistency, robustness, and smoothness. In scenarios where distributional information about predictions is available, a strong expected performance is required. Typically, the design of these algorithms involves a natural tradeoff between consistency and robustness, and previous works aimed to achieve Pareto-optimal tradeoffs for specific problems. However, in some settings, this comes at the expense of smoothness. This paper demonstrates that certain problems involve multiple tradeoffs between consistency, robustness, smoothness, and average performance.

==> conclusion.tex <==
\section{CONCLUSION}

Achieving Pareto-optimal tradeoffs between consistency and robustness in the design of learning-augmented algorithms is a challenging and highly interesting question. However, the absence of smoothness guarantees strongly limits the applicability of these algorithms in practical scenarios, where predictions are rarely perfectly accurate.

In the cases of the \textit{line search} and \textit{one-max search} problems, we demonstrated that by introducing randomization into brittle algorithms that exhibit Pareto-optimal consistency-robustness tradeoffs, we can establish smoothness guarantees. This approach consequently reveals an additional tradeoff between consistency and smoothness.

On the other hand, in the ski rental problem, we interestingly find that the Pareto-optimal tradeoff between consistency and robustness can be achieved by multiple algorithms, each exhibiting a different level of smoothness. However, improving smoothness results in a degradation of the average-case performance of the algorithm, hence showing another tradeoff between these criteria.

Our work highlights that, although learning-augmented algorithms have been extensively studied in the last few years, many of their aspects might have not been examined in the existing literature. In particular, we showed that the mutual dependencies among the various criteria involve additional tradeoffs and limitations, opening new research questions in the field. Potential avenues for follow-up research include
\begin{itemize}
    \item establishing Pareto-optimal fronts on the consistency, robustness, and smoothness, for example on deterministic algorithms,
    \item further exploration regarding how improvements in these criteria influence average-case performance under reasonable stochastic assumptions on prediction errors.
\end{itemize}  



